The Swift Deep Galactic Plane Survey (DGPS) Phase-I Catalog

The \textit{Swift} Deep Galactic Plane Survey is a \textit{Swift} Key Project consisting of 380 tiled pointings covering 40 deg$^{2}$ of the Galactic Plane between longitude $10$\,$<$\,$|l|$\,$<$\,$30$ deg and latitude $|b|$\,$<$\,$0.5$ deg. Each pointing has a $5$ ks exposure, yielding a total of 1.9 Ms spread across the entire survey footprint. Phase-I observations were carried out between March 2017 and May 2021. The Survey is complete to depth $L_X$\,$>$\,$10^{34}$ erg s$^{-1}$ to the edge of the Galaxy. The main Survey goal is to produce a rich sample of new X-ray sources and transients, while also covering a broad discovery space. Here, we introduce the Survey strategy and present a catalog of sources detected during Phase-I observations. In total, we identify 928 X-ray sources, of which 348 are unique to our X-ray catalog. We report on the characteristics of sources in our catalog and highlight sources newly classified and published by the DGPS team.

==> meerkat_stuff.tex <==


\subsection{Radio to X-ray flux ratios}

\textcolor{red}{FINISH THIS DISCUSSION... https://core.ac.uk/download/pdf/9562624.pdf and https://ui.adsabs.harvard.edu/abs/2018MNRAS.479.2481S/abstract}

Using the 57 MeerKAT counteparts to our sources we explore the X-ray to radio flux ratios to provide a first cut on source classification. Following \citet{Maccarone2012}, we display the 1.4 GHz radio flux density in mJy and the $0.3-10$ keV X-ray flux in erg cm$^{-2}$ s$^{-1}$ in Figure \ref{XXX}. The flux ratio $F_R/F_X$ is therefore in units of Hz$^{-1}$, where $F_R$ has been first converted to erg s$^{-1}$ Hz$^{-1}$. 

%Source with Fr/Fx~1e-10 could be AGN... 

 \begin{figure} 
\centering
\includegraphics[width=\columnwidth]{figs/Meerkat_result.pdf}
%\includegraphics[width=\columnwidth]{figs/Rate_logN-logS.pdf}
\caption{X-ray flux versus the ratio of the radio flux density to the X-ray flux for MeerKAT GPS counterparts to DGPS sources. The colorbar indicates the radio flux density of the sources in mJy.
}
\label{fig: radioflux}
\end{figure}


==> tables.tex <==
\section{List of DGPS Observations}

Here we provide a list of all \textit{Swift} observations comprising the DGPS Phase-I Survey footprint.

\startlongtable
\begin{deluxetable*}{lccc}
\tablecaption{List of \textit{Swift} Target IDs comprising the DGPS Phase-I observations. 
\label{tab: DGPS_obs_list}}
\tablehead{\colhead{Target ID} & \colhead{Name} & \colhead{RA (J2000)}  & \colhead{Dec (J2000)}}
\startdata
87317     & SGPS J1612.6-5139 & 243.157917 & -51.644556 \\
87318     & SGPS J1837.8-0602 & 279.449167 & -6.025556  \\
87319     & SGPS J1840.3-0560 & 280.085    & -5.995611  \\
87320     & SGPS J1841.5-0526 & 280.376667 & -5.432528  \\
87321     & SGPS J1842.7-0452 & 280.6675   & -4.869361  \\
87322     & SGPS J1844.3-0329 & 281.075833 & -3.476556  \\
87323     & SGPS J1604.2-5206 & 241.04375  & -52.093389 \\
87324     & SGPS J1604.6-5224 & 241.147917 & -52.403583 \\
87325     & SGPS J1605.7-5153 & 241.4275   & -51.882694 \\
87326     & SGPS J1606.1-5212 & 241.53375  & -52.192556 \\
87327     & SGPS J1606.6-5230 & 241.64125  & -52.502333 \\
87328     & SGPS J1607.2-5140 & 241.807917 & -51.670778 \\
87329     & SGPS J1607.7-5159 & 241.91625  & -51.980306 \\
87330     & SGPS J1608.1-5217 & 242.025833 & -52.289722 \\
87331     & SGPS J1608.7-5127 & 242.184583 & -51.457639 \\
87332     & SGPS J1609.2-5146 & 242.295    & -51.766806 \\
87333     & SGPS J1609.6-5205 & 242.407083 & -52.075861 \\
87334     & SGPS J1610.2-5115 & 242.557917 & -51.243306 \\
87335     & SGPS J1610.7-5133 & 242.670417 & -51.552111 \\
87336     & SGPS J1611.1-5152 & 242.784167 & -51.860806 \\
87337     & SGPS J1611.7-5102 & 242.9275   & -51.027778 \\
87338     & SGPS J1612.2-5120 & 243.042083 & -51.336222 \\
87339     & SGPS J1613.2-5049 & 243.29375  & -50.811083 \\
87340     & SGPS J1613.6-5107 & 243.41     & -51.119167 \\
87341     & SGPS J1614.1-5126 & 243.527917 & -51.427139 \\
87342     & SGPS J1614.6-5036 & 243.656667 & -50.59325  \\
87343     & SGPS J1615.1-5054 & 243.775    & -50.900972 \\
87344     & SGPS J1615.6-5113 & 243.894583 & -51.208583 \\
87345     & SGPS J1616.1-5022 & 244.01625  & -50.374306 \\
87346     & SGPS J1616.5-5041 & 244.13625  & -50.681667 \\
87347     & SGPS J1617.0-5059 & 244.257917 & -50.988889 \\
87348     & SGPS J1617.5-5009 & 244.3725   & -50.15425  \\
87349     & SGPS J1618.0-5028 & 244.494167 & -50.461222 \\
87350     & SGPS J1618.5-5046 & 244.6175   & -50.768083 \\
87351     & SGPS J1618.9-4956 & 244.725417 & -49.933111 \\
87352     & SGPS J1619.4-5014 & 244.84875  & -50.239722 \\
87353     & SGPS J1619.9-5033 & 244.97375  & -50.546194 \\
87354     & SGPS J1620.3-4943 & 245.075417 & -49.710889 \\
87355     & SGPS J1620.8-5001 & 245.200417 & -50.017139 \\
87356     & SGPS J1621.3-5019 & 245.327083 & -50.323222 \\
87357     & SGPS J1621.7-4929 & 245.421667 & -49.487639 \\
87358     & SGPS J1622.2-4948 & 245.548333 & -49.7935   \\
87359     & SGPS J1622.7-5006 & 245.676667 & -50.099222 \\
87360     & SGPS J1623.1-4916 & 245.765    & -49.263361 \\
87361     & SGPS J1623.6-4934 & 245.893333 & -49.568833 \\
87362     & SGPS J1624.1-4952 & 246.023333 & -49.874167 \\
87363     & SGPS J1624.4-4902 & 246.105417 & -49.038056 \\
87364     & SGPS J1624.9-4921 & 246.235    & -49.343139 \\
87365     & SGPS J1625.5-4939 & 246.36625  & -49.648083 \\
87366     & SGPS J1625.8-4849 & 246.4425   & -48.81175  \\
87367     & SGPS J1626.3-4907 & 246.57375  & -49.116472 \\
87368     & SGPS J1626.8-4925 & 246.706667 & -49.421028 \\
87369     & SGPS J1627.1-4835 & 246.77625  & -48.584472 \\
87370     & SGPS J1627.6-4853 & 246.909167 & -48.888806 \\
87371     & SGPS J1628.2-4912 & 247.043333 & -49.192972 \\
87372     & SGPS J1629.0-4840 & 247.241667 & -48.660167 \\
87373     & SGPS J1629.5-4858 & 247.3775   & -48.963972 \\
87374     & SGPS J1835.5-0709 & 278.862917 & -7.1505    \\
87375     & SGPS J1836.0-0652 & 279.009583 & -6.869333  \\
87376     & SGPS J1836.1-0725 & 279.035    & -7.41725   \\
87377     & SGPS J1836.6-0635 & 279.15625  & -6.588111  \\
87378     & SGPS J1836.7-0708 & 279.181667 & -7.136028  \\
87379     & SGPS J1837.2-0618 & 279.302917 & -6.306861  \\
87380     & SGPS J1837.3-0651 & 279.328333 & -6.85475   \\
87381     & SGPS J1837.4-0724 & 279.354167 & -7.402639  \\
87382     & SGPS J1837.9-0634 & 279.474583 & -6.573417  \\
87383     & SGPS J1838.0-0707 & 279.500417 & -7.121306  \\
87384     & SGPS J1838.4-0545 & 279.595    & -5.744194  \\
87385     & SGPS J1838.5-0618 & 279.620833 & -6.292056  \\
87386     & SGPS J1838.6-0650 & 279.647083 & -6.839944  \\
87387     & SGPS J1839.0-0528 & 279.740833 & -5.462806  \\
87388     & SGPS J1839.1-0601 & 279.767083 & -6.010667  \\
87389     & SGPS J1839.2-0634 & 279.793333 & -6.558528  \\
87390     & SGPS J1839.5-0511 & 279.886667 & -5.181361  \\
87392     & SGPS J1839.8-0617 & 279.939167 & -6.277083  \\
87393     & SGPS J1840.1-0454 & 280.0325   & -4.899889  \\
87395     & SGPS J1840.7-0437 & 280.177917 & -4.618389  \\
87396     & SGPS J1840.8-0510 & 280.204583 & -5.16625   \\
87397     & SGPS J1840.9-0543 & 280.230833 & -5.714083  \\
87398     & SGPS J1841.3-0420 & 280.323333 & -4.336861  \\
87400     & SGPS J1841.9-0403 & 280.46875  & -4.055278  \\
87402     & SGPS J1842.1-0509 & 280.522083 & -5.150972  \\
87403     & SGPS J1842.5-0346 & 280.61375  & -3.773694  \\
87405     & SGPS J1843.0-0330 & 280.75875  & -3.492056  \\
87407     & SGPS J1843.3-0435 & 280.8125   & -4.587722  \\
87408     & SGPS J1843.6-0313 & 280.90375  & -3.210417  \\
87410     & SGPS J1843.8-0418 & 280.957917 & -4.306056  \\
87411     & SGPS J1844.2-0256 & 281.04875  & -2.928722  \\
87412     & SGPS J1844.4-0401 & 281.102917 & -4.024361  \\
87413     & SGPS J1844.8-0239 & 281.19375  & -2.647028  \\
87414     & SGPS J1844.9-0312 & 281.220833 & -3.194833  \\
87415     & SGPS J1845.0-0345 & 281.247917 & -3.742667  \\
87416     & SGPS J1845.5-0255 & 281.365417 & -2.913111  \\
87417     & SGPS J1845.6-0328 & 281.3925   & -3.460917  \\
87418     & SGPS J1846.0-0238 & 281.510417 & -2.631389  \\
87419     & SGPS J1846.1-0311 & 281.5375   & -3.179194  \\
87420     & SGPS J1846.7-0254 & 281.682083 & -2.897417  \\
87421     & SGPS J1822.4-1352 & 275.5925   & -13.868167 \\
87422     & SGPS J1659.8-4226 & 254.938333 & -42.425556 \\
87423     & SGPS J1820.5-1442 & 275.13125  & -14.706417 \\
87424     & SGPS J1700.2-4153 & 255.0425   & -41.882583 \\
87425     & SGPS J1701.2-4138 & 255.304167 & -41.633    \\
87426     & SGPS J1818.7-1606 & 274.68375  & -16.091972 \\
87427     & SGPS J1810.5-1943 & 272.616667 & -19.708417 \\
87428     & SGPS J1714.1-3820 & 258.526667 & -38.338167 \\
87429     & SGPS J1709.0-4010 & 257.241667 & -40.160833 \\
87430     & SGPS J1642.2-4637 & 250.555    & -46.624194 \\
87431     & SGPS J1641.0-4652 & 250.249583 & -46.862    \\
87432     & SGPS J1639.8-4706 & 249.941667 & -47.099    \\
87433     & SGPS J1638.5-4720 & 249.63125  & -47.335167 \\
87434     & SGPS J1637.3-4734 & 249.317917 & -47.5705   \\
87435     & SGPS J1636.0-4748 & 249.001667 & -47.804972 \\
87436     & SGPS J1634.7-4802 & 248.682917 & -48.038583 \\
87437     & SGPS J1633.4-4816 & 248.360833 & -48.271278 \\
87438     & SGPS J1632.1-4830 & 248.035833 & -48.503111 \\
87439     & SGPS J1630.8-4844 & 247.708333 & -48.734    \\
87440     & SGPS J1648.1-4435 & 252.02625  & -44.585722 \\
87441     & SGPS J1647.0-4450 & 251.737917 & -44.827333 \\
87442     & SGPS J1645.8-4504 & 251.4475   & -45.06825  \\
87443     & SGPS J1644.6-4519 & 251.155    & -45.308389 \\
87444     & SGPS J1643.4-4533 & 250.859583 & -45.547778 \\
87445     & SGPS J1642.2-4547 & 250.561667 & -45.786389 \\
87446     & SGPS J1641.0-4601 & 250.26125  & -46.024222 \\
87447     & SGPS J1639.8-4616 & 249.957917 & -46.26125  \\
87448     & SGPS J1638.6-4630 & 249.6525   & -46.497472 \\
87449     & SGPS J1637.4-4644 & 249.344167 & -46.732861 \\
87450     & SGPS J1636.1-4658 & 249.032917 & -46.967417 \\
87451     & SGPS J1634.9-4712 & 248.719167 & -47.201111 \\
87452     & SGPS J1633.6-4726 & 248.4025   & -47.433944 \\
87453     & SGPS J1632.3-4740 & 248.082917 & -47.665861 \\
87454     & SGPS J1631.0-4754 & 247.760833 & -47.896917 \\
87455     & SGPS J1629.7-4808 & 247.435417 & -48.127028 \\
87456     & SGPS J1628.4-4821 & 247.1075   & -48.356222 \\
87457     & SGPS J1649.9-4438 & 252.464167 & -44.64075  \\
87458     & SGPS J1648.7-4453 & 252.177917 & -44.8835   \\
87459     & SGPS J1647.6-4508 & 251.88875  & -45.1255   \\
87460     & SGPS J1646.4-4522 & 251.5975   & -45.366778 \\
87461     & SGPS J1645.2-4536 & 251.30375  & -45.607333 \\
87462     & SGPS J1644.0-4551 & 251.0075   & -45.847083 \\
87463     & SGPS J1642.8-4605 & 250.70875  & -46.086083 \\
87464     & SGPS J1641.6-4619 & 250.407083 & -46.324306 \\
87465     & SGPS J1640.4-4634 & 250.102917 & -46.561722 \\
87466     & SGPS J1639.2-4648 & 249.79625  & -46.798333 \\
87467     & SGPS J1637.9-4702 & 249.486667 & -47.034111 \\
87468     & SGPS J1636.7-4716 & 249.174583 & -47.269056 \\
87469     & SGPS J1635.4-4730 & 248.859583 & -47.503139 \\
87470     & SGPS J1634.2-4744 & 248.541667 & -47.736333 \\
87471     & SGPS J1632.9-4758 & 248.22125  & -47.968667 \\
87472     & SGPS J1631.6-4812 & 247.8975   & -48.200083 \\
87473     & SGPS J1630.3-4826 & 247.57125  & -48.430583 \\
87474     & SGPS J1827.3-1211 & 276.829167 & -12.176833 \\
87475     & SGPS J1827.9-1154 & 276.979583 & -11.8965   \\
87476     & SGPS J1828.5-1137 & 277.13     & -11.616139 \\
87477     & SGPS J1829.1-1120 & 277.28     & -11.335667 \\
87478     & SGPS J1829.7-1103 & 277.43     & -11.055139 \\
87479     & SGPS J1830.3-1046 & 277.579167 & -10.774528 \\
87480     & SGPS J1830.9-1030 & 277.72875  & -10.493861 \\
87481     & SGPS J1831.5-1013 & 277.8775   & -10.213139 \\
87482     & SGPS J1832.1-0956 & 278.02625  & -9.932333  \\
87483     & SGPS J1832.7-0939 & 278.174583 & -9.651472  \\
87484     & SGPS J1833.3-0922 & 278.322917 & -9.370556  \\
87485     & SGPS J1833.9-0905 & 278.470833 & -9.089583  \\
87486     & SGPS J1834.5-0849 & 278.618333 & -8.808556  \\
87487     & SGPS J1835.1-0832 & 278.765833 & -8.527472  \\
87488     & SGPS J1835.7-0815 & 278.913333 & -8.246333  \\
87489     & SGPS J1836.2-0758 & 279.060417 & -7.965139  \\
87490     & SGPS J1836.8-0741 & 279.2075   & -7.683917  \\
87491     & SGPS J1825.3-1155 & 276.332917 & -11.921083 \\
87492     & SGPS J1825.9-1138 & 276.484167 & -11.641056 \\
87493     & SGPS J1826.5-1122 & 276.634583 & -11.360917 \\
87494     & SGPS J1827.1-1105 & 276.785    & -11.080694 \\
87495     & SGPS J1827.7-1048 & 276.935    & -10.800417 \\
87496     & SGPS J1828.3-1031 & 277.085    & -10.520056 \\
87497     & SGPS J1828.9-1014 & 277.234583 & -10.239611 \\
87498     & SGPS J1829.5-0958 & 277.38375  & -9.959111  \\
87499     & SGPS J1830.1-0941 & 277.532917 & -9.678528  \\
87500     & SGPS J1830.7-0924 & 277.681667 & -9.397889  \\
87501     & SGPS J1831.3-0907 & 277.83     & -9.117167  \\
87502     & SGPS J1831.9-0850 & 277.978333 & -8.836389  \\
87503     & SGPS J1832.5-0833 & 278.12625  & -8.555556  \\
87504     & SGPS J1833.1-0816 & 278.274167 & -8.274667  \\
87505     & SGPS J1833.7-0760 & 278.421667 & -7.993694  \\
87506     & SGPS J1834.3-0743 & 278.56875  & -7.712694  \\
87507     & SGPS J1834.9-0726 & 278.715833 & -7.431639  \\
87508     & SGPS J1826.0-1211 & 276.505417 & -12.189111 \\
87509     & SGPS J1826.6-1155 & 276.65625  & -11.908972 \\
87510     & SGPS J1827.2-1138 & 276.807083 & -11.62875  \\
87511     & SGPS J1827.8-1121 & 276.9575   & -11.348472 \\
87512     & SGPS J1828.4-1104 & 277.1075   & -11.068083 \\
87513     & SGPS J1829.0-1047 & 277.257083 & -10.787639 \\
87514     & SGPS J1829.6-1030 & 277.406667 & -10.507139 \\
87515     & SGPS J1830.2-1014 & 277.555833 & -10.226528 \\
87516     & SGPS J1830.8-0957 & 277.705    & -9.945889  \\
87517     & SGPS J1831.4-0940 & 277.85375  & -9.665167  \\
87518     & SGPS J1832.0-0923 & 278.002083 & -9.384361  \\
87519     & SGPS J1832.6-0906 & 278.150417 & -9.103528  \\
87520     & SGPS J1833.2-0849 & 278.298333 & -8.822611  \\
87521     & SGPS J1833.8-0832 & 278.44625  & -8.541639  \\
87522     & SGPS J1834.4-0816 & 278.59375  & -8.260639  \\
87523     & SGPS J1835.0-0759 & 278.740833 & -7.979556  \\
87524     & SGPS J1835.6-0742 & 278.887917 & -7.698417  \\
3110725   & SGPS J1817.4-1606 & 274.354481 & -16.10144  \\
3110726   & SGPS J1818.0-1549 & 274.510689 & -15.822653 \\
3110727   & SGPS J1818.7-1533 & 274.666468 & -15.543755 \\
3110728   & SGPS J1819.3-1516 & 274.821825 & -15.264747 \\
3110729   & SGPS J1819.9-1459 & 274.976769 & -14.985633 \\
3110730   & SGPS J1821.1-1426 & 275.285457 & -14.427094 \\
3110731   & SGPS J1821.8-1409 & 275.439216 & -14.147673 \\
3110732   & SGPS J1823.0-1335 & 275.745612 & -13.588542 \\
3110733   & SGPS J1823.6-1319 & 275.898264 & -13.308835 \\
3110734   & SGPS J1824.2-1302 & 276.050564 & -13.029038 \\
3110735   & SGPS J1824.8-1245 & 276.202521 & -12.749152 \\
3110736   & SGPS J1825.4-1228 & 276.354142 & -12.469179 \\
3110737   & SGPS J1815.5-1623 & 273.867886 & -16.388824 \\
3110738   & SGPS J1816.1-1607 & 274.025009 & -16.110397 \\
3110739   & SGPS J1816.7-1550 & 274.181683 & -15.831852 \\
3110740   & SGPS J1817.4-1533 & 274.337918 & -15.553191 \\
3110741   & SGPS J1818.0-1516 & 274.493723 & -15.274416 \\
3110742   & SGPS J1818.6-1460 & 274.649106 & -14.995529 \\
3110743   & SGPS J1819.2-1443 & 274.804077 & -14.716534 \\
3110744   & SGPS J1819.8-1426 & 274.958645 & -14.437432 \\
3110745   & SGPS J1820.5-1409 & 275.112818 & -14.158226 \\
3110746   & SGPS J1821.1-1353 & 275.266604 & -13.878917 \\
3110747   & SGPS J1821.7-1336 & 275.420013 & -13.599509 \\
3110748   & SGPS J1822.3-1319 & 275.573053 & -13.320003 \\
3110749   & SGPS J1822.9-1302 & 275.725732 & -13.040402 \\
3110750   & SGPS J1823.5-1246 & 275.878058 & -12.760707 \\
3110751   & SGPS J1824.1-1229 & 276.03004  & -12.480922 \\
3110752   & SGPS J1824.7-1212 & 276.181687 & -12.201048 \\
3110753   & SGPS J1817.5-1639 & 274.371135 & -16.64969  \\
3110754   & SGPS J1818.1-1622 & 274.527748 & -16.370891 \\
3110755   & SGPS J1819.4-1549 & 274.839665 & -15.81296  \\
3110756   & SGPS J1820.0-1532 & 274.994986 & -15.533834 \\
3110757   & SGPS J1820.6-1515 & 275.149896 & -15.254603 \\
3110758   & SGPS J1821.2-1459 & 275.304401 & -14.97527  \\
3110759   & SGPS J1821.8-1442 & 275.458512 & -14.695837 \\
3110760   & SGPS J1822.4-1425 & 275.612236 & -14.416307 \\
3110761   & SGPS J1823.1-1408 & 275.765583 & -14.136681 \\
3110762   & SGPS J1823.7-1351 & 275.918561 & -13.856963 \\
3110763   & SGPS J1824.3-1335 & 276.071179 & -13.577153 \\
3110764   & SGPS J1824.9-1318 & 276.223445 & -13.297255 \\
3110765   & SGPS J1825.5-1301 & 276.375366 & -13.01727  \\
3110766   & SGPS J1826.1-1244 & 276.526953 & -12.737202 \\
3110767   & SGPS J1826.7-1227 & 276.678212 & -12.457051 \\
3110768   & SGPS J1708.0-4025 & 256.993409 & -40.414684 \\
3110769   & SGPS J1707.0-4040 & 256.743374 & -40.668011 \\
3110770   & SGPS J1706.0-4055 & 256.491435 & -40.920794 \\
3110771   & SGPS J1705.0-4110 & 256.237563 & -41.173024 \\
3110772   & SGPS J1703.9-4125 & 255.981732 & -41.424693 \\
3110773   & SGPS J1702.9-4141 & 255.723911 & -41.67579  \\
3110774   & SGPS J1701.9-4156 & 255.464073 & -41.926307 \\
3110775   & SGPS J1700.8-4211 & 255.202189 & -42.176233 \\
3110776   & SGPS J1658.7-4240 & 254.672165 & -42.674275 \\
3110777   & SGPS J1657.6-4255 & 254.403965 & -42.92237  \\
3110778   & SGPS J1656.5-4310 & 254.133598 & -43.169834 \\
3110779   & SGPS J1655.4-4325 & 253.861035 & -43.416656 \\
3110780   & SGPS J1654.3-4340 & 253.586243 & -43.662826 \\
3110781   & SGPS J1653.2-4354 & 253.309192 & -43.908332 \\
3110782   & SGPS J1652.1-4409 & 253.029849 & -44.153163 \\
3110783   & SGPS J1651.0-4424 & 252.748182 & -44.397307 \\
3110784   & SGPS J1708.3-3952 & 257.077905 & -39.870019 \\
3110785   & SGPS J1707.3-4007 & 256.830205 & -40.123529 \\
3110786   & SGPS J1706.3-4023 & 256.580644 & -40.376503 \\
3110787   & SGPS J1705.3-4038 & 256.329195 & -40.628932 \\
3110788   & SGPS J1704.3-4053 & 256.075831 & -40.880806 \\
3110789   & SGPS J1703.3-4108 & 255.820525 & -41.132116 \\
3110790   & SGPS J1702.3-4123 & 255.563248 & -41.382853 \\
3110791   & SGPS J1659.1-4208 & 254.779315 & -42.13153  \\
3110792   & SGPS J1658.1-4223 & 254.513874 & -42.379878 \\
3110793   & SGPS J1657.0-4238 & 254.246318 & -42.627603 \\
3110794   & SGPS J1655.9-4252 & 253.976617 & -42.874696 \\
3110795   & SGPS J1654.8-4307 & 253.704743 & -43.121145 \\
3110796   & SGPS J1653.7-4322 & 253.430663 & -43.36694  \\
3110797   & SGPS J1652.6-4337 & 253.154347 & -43.61207  \\
3110798   & SGPS J1651.5-4351 & 252.875763 & -43.856524 \\
3110799   & SGPS J1650.4-4406 & 252.59488  & -44.10029  \\
3110800   & SGPS J1649.2-4421 & 252.311665 & -44.343357 \\
3110801   & SGPS J1710.6-4012 & 257.65337  & -40.196659 \\
3110802   & SGPS J1709.6-4027 & 257.406634 & -40.451395 \\
3110803   & SGPS J1708.6-4042 & 257.158031 & -40.705607 \\
3110804   & SGPS J1707.6-4058 & 256.907534 & -40.959287 \\
3110805   & SGPS J1706.6-4113 & 256.655114 & -41.212425 \\
3110806   & SGPS J1705.6-4128 & 256.400745 & -41.465013 \\
3110807   & SGPS J1704.6-4143 & 256.144398 & -41.717041 \\
3110808   & SGPS J1703.5-4158 & 255.886043 & -41.9685   \\
3110809   & SGPS J1702.5-4213 & 255.625652 & -42.219381 \\
3110810   & SGPS J1701.5-4228 & 255.363195 & -42.469673 \\
3110811   & SGPS J1700.4-4243 & 255.098642 & -42.719367 \\
3110812   & SGPS J1659.3-4258 & 254.831963 & -42.968452 \\
3110813   & SGPS J1658.3-4313 & 254.563128 & -43.216918 \\
3110814   & SGPS J1657.2-4328 & 254.292104 & -43.464755 \\
3110815   & SGPS J1656.1-4343 & 254.01886  & -43.711952 \\
3110816   & SGPS J1655.0-4358 & 253.743366 & -43.958498 \\
3110817   & SGPS J1653.9-4412 & 253.465587 & -44.204381 \\
3110818   & SGPS J1652.7-4427 & 253.185493 & -44.449591 \\
3110819   & SGPS J1651.6-4442 & 252.903049 & -44.694117 \\
3110820   & SGPS J1650.5-4456 & 252.618222 & -44.937945 \\
3110821   & SGPS J1649.3-4511 & 252.330979 & -45.181065 \\
3110822   & SGPS J1648.2-4525 & 252.041285 & -45.423464 \\
3110823   & SGPS J1647.0-4540 & 251.749105 & -45.66513  \\
3110824   & SGPS J1645.8-4554 & 251.454405 & -45.906051 \\
3110825   & SGPS J1644.6-4609 & 251.157149 & -46.146212 \\
3110826   & SGPS J1643.4-4623 & 250.857302 & -46.385602 \\
3110839   & SGPS J1807.8-2016 & 271.95337  & -20.268196 \\
3110844   & SGPS J1811.1-1853 & 272.766698 & -18.882647 \\
3110845   & SGPS J1811.7-1836 & 272.927721 & -18.605109 \\
3110846   & SGPS J1812.4-1820 & 273.088219 & -18.327435 \\
3110847   & SGPS J1813.0-1803 & 273.248202 & -18.049627 \\
3110848   & SGPS J1813.6-1746 & 273.40768  & -17.771688 \\
3110849   & SGPS J1814.3-1730 & 273.566663 & -17.49362  \\
3110850   & SGPS J1814.9-1713 & 273.725161 & -17.215427 \\
3110851   & SGPS J1815.5-1656 & 273.883182 & -16.937109 \\
3110852   & SGPS J1816.2-1640 & 274.040736 & -16.658671 \\
3110853   & SGPS J1816.8-1623 & 274.197833 & -16.380114 \\
3110855   & SGPS J1822.4-1352 & 275.592599 & -13.868155 \\
3110856   & SGPS J1807.1-1960 & 271.780231 & -19.996438 \\
3110857   & SGPS J1807.8-1943 & 271.944044 & -19.719784 \\
3110858   & SGPS J1808.4-1927 & 272.107283 & -19.442978 \\
3110859   & SGPS J1809.1-1910 & 272.269958 & -19.166021 \\
3110860   & SGPS J1809.7-1853 & 272.43208  & -18.888919 \\
3110861   & SGPS J1810.4-1837 & 272.593657 & -18.611671 \\
3110862   & SGPS J1811.0-1820 & 272.754702 & -18.334283 \\
3110863   & SGPS J1811.7-1803 & 272.915222 & -18.056756 \\
3110864   & SGPS J1812.3-1747 & 273.075229 & -17.779092 \\
3110865   & SGPS J1812.9-1730 & 273.234731 & -17.501296 \\
3110866   & SGPS J1813.6-1713 & 273.393738 & -17.223368 \\
3110867   & SGPS J1814.2-1657 & 273.552261 & -16.945311 \\
3110868   & SGPS J1814.8-1640 & 273.710307 & -16.667129 \\
3110869   & SGPS J1809.2-2016 & 272.290884 & -20.262808 \\
3110870   & SGPS J1809.8-1959 & 272.454076 & -19.985686 \\
3110871   & SGPS J1810.5-1943 & 272.616702 & -19.708419 \\
3110872   & SGPS J1811.1-1926 & 272.778773 & -19.43101  \\
3110873   & SGPS J1811.8-1909 & 272.940299 & -19.153462 \\
3110874   & SGPS J1812.4-1853 & 273.10129  & -18.875777 \\
3110875   & SGPS J1813.0-1836 & 273.261756 & -18.597958 \\
3110876   & SGPS J1813.7-1819 & 273.421707 & -18.320008 \\
3110877   & SGPS J1814.3-1803 & 273.581153 & -18.041929 \\
3110878   & SGPS J1815.0-1746 & 273.740103 & -17.763724 \\
3110879   & SGPS J1815.6-1729 & 273.898566 & -17.485394 \\
3110880   & SGPS J1816.2-1712 & 274.056553 & -17.206944 \\
3110881   & SGPS J1816.9-1656 & 274.214073 & -16.928375 \\
3110882   & SGPS J1818.7-1606 & 274.683921 & -16.09198  \\
3110883   & SGPS J1719.4-3720 & 259.854803 & -37.335469 \\
3110884   & SGPS J1718.5-3736 & 259.625603 & -37.594665 \\
3110885   & SGPS J1717.6-3751 & 259.394802 & -37.853415 \\
3110886   & SGPS J1716.6-3807 & 259.162376 & -38.111711 \\
3110887   & SGPS J1715.7-3822 & 258.928302 & -38.369546 \\
3110888   & SGPS J1714.8-3838 & 258.692556 & -38.626912 \\
3110889   & SGPS J1713.8-3853 & 258.455113 & -38.883802 \\
3110890   & SGPS J1712.9-3908 & 258.215948 & -39.140207 \\
3110891   & SGPS J1711.9-3924 & 257.975037 & -39.39612  \\
3110892   & SGPS J1710.9-3939 & 257.732353 & -39.651533 \\
3110893   & SGPS J1710.0-3954 & 257.487871 & -39.906437 \\
3110894   & SGPS J1709.0-4010 & 257.241565 & -40.160824 \\
3110895   & SGPS J1659.8-4226 & 254.93823  & -42.42556  \\
3110896   & SGPS J1717.8-3718 & 259.45819  & -37.307238 \\
3110897   & SGPS J1716.9-3734 & 259.227704 & -37.56566  \\
3110898   & SGPS J1716.0-3749 & 258.995605 & -37.823627 \\
3110899   & SGPS J1715.0-3805 & 258.761872 & -38.08113  \\
3110900   & SGPS J1714.1-3820 & 258.526478 & -38.338162 \\
3110901   & SGPS J1713.2-3836 & 258.289402 & -38.594715 \\
3110902   & SGPS J1712.2-3851 & 258.050618 & -38.850781 \\
3110903   & SGPS J1711.2-3906 & 257.810102 & -39.106353 \\
3110904   & SGPS J1710.3-3922 & 257.567828 & -39.361422 \\
3110905   & SGPS J1709.3-3937 & 257.323771 & -39.61598  \\
3110906   & SGPS J1701.2-4138 & 255.303974 & -41.633008 \\
3110907   & SGPS J1700.2-4153 & 255.042672 & -41.88257  \\
3110908   & SGPS J1720.1-3737 & 260.023806 & -37.622332 \\
3110909   & SGPS J1719.2-3753 & 259.794314 & -37.881853 \\
3110910   & SGPS J1718.3-3808 & 259.56321  & -38.14093  \\
3110911   & SGPS J1717.3-3824 & 259.330468 & -38.399556 \\
3110912   & SGPS J1716.4-3839 & 259.096065 & -38.657724 \\
3110913   & SGPS J1715.4-3855 & 258.859977 & -38.915425 \\
3110914   & SGPS J1714.5-3910 & 258.622178 & -39.172652 \\
3110915   & SGPS J1713.5-3926 & 258.382644 & -39.429397 \\
3110916   & SGPS J1712.6-3941 & 258.141348 & -39.685652 \\
3110917   & SGPS J1711.6-3956 & 257.898266 & -39.941409 \\
3110990   & SGPS J1808.5-1959 & 272.117165 & -19.99138  \\
3110991   & SGPS J1809.1-1943 & 272.280385 & -19.714415 \\
3110992   & SGPS J1809.8-1926 & 272.443041 & -19.437302 \\
3110993   & SGPS J1810.4-1910 & 272.605142 & -19.160045
\enddata

\end{deluxetable*}


